QCD in magnetic field, Landau levels and double-life of unbroken center-symmetry

We study the thermal confinement/deconfinement and non-thermal quantum phase transitions or rapid cross-overs in QCD and QCD-like theories in external magnetic fields. At large magnetic fields, while the contribution of gauge fluctuations to Wilson-line potential remains unaltered at one-loop order, the contribution of fermions effectively becomes two lower dimensional and is enhanced by the density of states of the lowest Landau level (LLL). In a spatial compactification and for heavy adjoint fermions, this enhancement leads to a calculable zero temperature quantum phase transition on R^3*S^1 driven by a competition between the center-destabilizing gauge contribution and center-stabilizing LLL fermions. We also show that at a (formal) asymptotically large magnetic field, the adjoint fermions with arbitrarily large but fixed mass stabilize the center symmetry. This is an exotic case of simultaneous non-decoupling of large mass fermions (due to the enhancement by the LLL density of states) and decoupling from the low energy effective field theory. This observation has important implications for both Hosotani mechanism, for which gauge symmetry "breaking" occurs, and large-N volume independence (Eguchi-Kawai reduction), for which gauge structure is never "broken". Despite sounding almost self-contradictory, we carefully explain the physical scales entering the problem, double-meaning of unbroken center symmetry and how a clash is avoided. We also identify, for both thermal and spatial compactification, the jump in magnetic susceptibility as an order parameter for the deconfinement transition. The predictions of our analysis are testable by using current lattice techniques.

==> JHEP3.cls.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% JHEP.cls 3.1.5 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% This file is Copyright JHEP 2005:  it can be freely distributed  but
%% NOT modified preserving its name, even in similar forms.
%% 
%% JHEP3.cls is a LaTeX2e class file used to typeset manuscripts in JHEP
%% style. It was written by F. Nesti as a (radical) modification of the
%% class `article.cls' from distribution 960601 of LaTeX2e.
%% 
%% For bugs, comments, suggestions email to jhep-eo@jhep.sissa.it
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  ***:to do  **?:question  ...:to choose  XXX:to delete  ???:unknown %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesClass{JHEP3} [2005/09/26 v3.1.4 LaTeX document class - F.N.]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\logo{\raisebox{-10.5\p@}{\hb@xt@85\p@{\special{psfile=JHEPlogo.eps}\hfil}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW SWITCHES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if@preprint\@preprinttrue		% DEFAULT IS PREPRINT!
\newif\if@draft   \@draftfalse			% DEFAULT IS NOT DRAFT
\newif\if@hyper   \@hypertrue			% DEFAULT IS HYPER
\newif\if@proc	  \@procfalse			% DEFAULT IS NOT PROC

%\newif\if@title\@titlefalse			%
\newif\if@author\@authorfalse			%
\newif\if@abstract\@abstractfalse		% FOR FRONTMATTER DECLARATIONS
\newif\if@keywords\@keywordsfalse		%
\newif\if@todotoc\@todotocfalse			%
\newif\if@rece\@recefalse			%
\newif\if@revi\@revifalse			%
\newif\if@acce\@accefalse			%
\newif\if@Jcopy\@Jcopyfalse			%
\newif\if@JHEP\@JHEPfalse			%
\newif\if@conf\@conffalse			%
\newif\if@Jspecialurl\@Jspecialurlfalse
\newif\ifpdf
\ifx\pdfoutput\undefined
\else
  \ifx\pdfoutput\relax
  \else
    \ifcase\pdfoutput
    \else
      \pdftrue
    \fi
  \fi
\fi
%%\newif\if@restonecol\@twocolumnfalse

\if@compatibility
    \setlength\paperheight {297mm}%		% DEFAULT FOR LATEX209 IS a4
    \setlength\paperwidth  {210mm}%
\else						% CHOSE PAPER:
\DeclareOption{a4paper}
   {\setlength\paperheight {297mm}%
    \setlength\paperwidth  {210mm}}
\DeclareOption{a5paper}{\@OImess{}}		% IGNORED a5
\DeclareOption{b5paper}{\@OImess{}}		% IGNORED b5
\DeclareOption{letterpaper}
   {\setlength\paperheight {11in}%
    \setlength\paperwidth  {8.5in}}
\DeclareOption{legalpaper}
   {\setlength\paperheight {14in}%
    \setlength\paperwidth  {8.5in}}
\DeclareOption{executivepaper}
   {\setlength\paperheight {10.5in}%
    \setlength\paperwidth  {7.25in}}
\DeclareOption{landscape}{\@OImess{}}		% IGNORED landscape
\fi

\newcommand\@ptsize{1}                          % DEFAULT SIZE IS 11 PT

\DeclareOption{proceedings}{\@preprintfalse\@proctrue
			   \renewcommand\@ptsize{1}% PROCS: 11 PT
			   \AtBeginDocument{\@todotocfalse}}


\DeclareOption{published}{%
\ifpdf
\JHEP@warnl{Option 'published' incompatible with 
pdf output, turning to dvi output}\pdffalse\pdfoutput=0\@preprintfalse
\else
\@preprintfalse%
\fi}


\DeclareOption{hyper}{\@hypertrue}	% HYPER IS 11 PT
%\DeclareOption{screen}{\@hypertrue}	% HYPER IS 11 PT
\DeclareOption{nohyper}{\@hyperfalse}	% PAPER IS ALSO 11 PT (v1.3)
\DeclareOption{paper}{\@hyperfalse}	% PAPER IS ALSO 11 PT
\DeclareOption{11pt}{\renewcommand\@ptsize{1}\ExecuteOptions{@FONT}}
\DeclareOption{12pt}{\renewcommand\@ptsize{2}\ExecuteOptions{@FONT}}
\if@compatibility\else                          % LATEX2.09 HAS NO 10PT 
\DeclareOption{10pt}{\renewcommand\@ptsize{0}\ExecuteOptions{@FONT}}% v1.4
\fi       				% CHOSEN TO FREE MEMORY LATER:
\DeclareOption{@FONT}{\if@preprint              % IF PREPRINT ALLOW ANY,
                        \else			% IF PROCEEDINGS OR PUBLISHED: 
%			\if@proc		% 
%			\renewcommand\@ptsize{0}\@NFmess{10pt}% ALWAYS 10PT
%			\else
			\renewcommand\@ptsize{1}\@NFmess{11pt}% ALWAYS 11PT
                        \fi%\fi
			}
                        
\if@compatibility\else
\DeclareOption{oneside}{\@twosidefalse \@mparswitchfalse}\fi
\DeclareOption{twoside}{\if@preprint\if@hyper\@OImess{ in hyper-mode}
				    \else\@twosidetrue\@mparswitchtrue\fi
			\else			% FOR PROCEED./PUBLIC.:
			\@OImess{ in published papers}
			\fi}
\DeclareOption{notoc}{\if@preprint		% to disable TOC
			\AtBeginDocument{\@todotocfalse}
			\else
			\if@proc\@OImess{ is automatic for proceedings}
			\else\@OImess{ in JHEP papers}\fi\fi}
\DeclareOption{draft}{\setlength\overfullrule{5pt}% EXTENDED DRAFT
	\newcount\hour\newcount\minute
	\hour=\time \divide\hour by60 \minute=\time
	{\multiply\hour by60 \global\advance\minute by-\hour}
	\edef\militarytime{\number\hour:\ifnum\minute<10 0\fi\number\minute}
	\let\old@eqnnum\@eqnnum
	\def\@eqnnum{\old@eqnnum\rlap{\kern\marginparsep
				\if@twocolumn\if@firstcolumn
				  \kern-2\marginparsep\kern-\columnwidth\
				  \llap\bgroup\else\bgroup\fi
				\else
				\if@twoside\ifodd\c@page
				  \kern-2\marginparsep\kern-\textwidth
				  \llap\bgroup\else\bgroup\fi
				\else\bgroup\fi				
				\fi
				\sf\scriptsize\@eqnlabel\egroup}%
				\gdef\@eqnlabel{}}
	\let\@eqnlabel\relax
	\def\math@note#1{\gdef\@eqnlabel{LAB: #1}}
	\def\norm@note#1#2{\special{}% SORRY AGAIN.
			 \ifinner{\ifdim\baselineskip=\z@% IN ARRAY..
					\baselineskip18\p@\fi%%
				\ifhmode%   ATTENTION TO RESTRICTED VMODE!
				\raisebox{.5\baselineskip}[\z@][\z@]{%
					\rlap{\sf\scriptsize #2}}%
				\else\vskip-\baselineskip%
				\raisebox{-.6\baselineskip}[\z@][\z@]{%
						\rlap{\sf\scriptsize #2}}%
				\fi}%
			 \else\marginpar{\raggedright\if@twoside\ifodd\c@page%
					\raggedleft\fi\fi\sf\scriptsize #1#2}%
			 \fi}%
	\AtBeginDocument{\newbox\drft@box\setbox\drft@box=\hbox{%
			\framebox[\textwidth]{\sf\small JHEP 3.1 DRAFT 
			\ttfamily(\cur@opt)\hfill\sf\bfseries\jobname\sf, 
			\today, \militarytime}}}
	\@drafttrue}

%\if@compatibility\else
%\DeclareOption{final}{\setlength\overfullrule{\z@}} % ***? NO FINAL?
%\fi
\DeclareOption{titlepage}{\@OImess{}}		% IGNORED
\if@compatibility\else
\DeclareOption{notitlepage}{\@OImess{}}		% IGNORED
\fi
\if@compatibility\else
\DeclareOption{onecolumn}{\@OImess{}}		% IGNORED
\fi
\DeclareOption{twocolumn}{\@OImess{}}		% IGNORED
\DeclareOption{leqno}{\@OImess{}}	%\input{leqno.clo}} IGNORED ...
\DeclareOption{fleqn}{\@OImess{}}	%\input{fleqn.clo}} IGNORED ...
\DeclareOption{openbib}{\@OImess{}}		% IGNORED


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MESSAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\JHEP@mess[1]{\typeout{Class JHEP Message: \protect#1.}}%
\newcommand\JHEP@warn[1]{\ClassWarning{JHEP}{#1}}
\newcommand\JHEP@warnl[1]{\ClassWarningNoLine{JHEP}{#1}}
\newcommand\JHEP@igno[1]{\JHEP@warn{IGNORED \protect#1}}
\newcommand\JHEP@ignol[1]{\JHEP@warnl{IGNORED \protect#1}}
\newcommand\@OImess[1]{\JHEP@ignol{OPTION '\CurrentOption'#1}}
\newcommand\@NFmess[1]{\JHEP@mess{Normalsize set to #1}}
\newcommand\@ENVwarn[1]{\JHEP@warn{Please use \protect#1 in place 
						of LaTeX environment}}
%%%%%%%%%%%%%%%%%%%%%%%%%% PROCESS OPTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ExecuteOptions{a4paper,oneside,hyper} %WERE ALSO 10pt,onecolumn
\ProcessOptions
%%%%%%%%%%%%%%%%%%%%%%%%%% REQUIRED PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{amssymb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%% START CODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{size1\@ptsize.clo}
\renewcommand{\baselinestretch}{1.1}\normalsize
\setlength\lineskip{1\p@}
\setlength\parindent{1.2\parindent}	% AT 12pt 1.5em BECOMES 1.8em=tocindent
\setlength\normallineskip{1\p@}
\setlength\parskip{0\p@ \@plus \p@}
\@lowpenalty   51
\@medpenalty  151
\@highpenalty 301
\widowpenalty 1000
\clubpenalty 1000

\setcounter{topnumber}{3}
\renewcommand\topfraction{.95} % default .7
\setcounter{bottomnumber}{1}
\renewcommand\bottomfraction{.6} %.2		% .6 ???***
\setcounter{totalnumber}{3}
\renewcommand\textfraction{.05}
\renewcommand\floatpagefraction{1}
\setcounter{dbltopnumber}{3}
\renewcommand\dbltopfraction{.7}
\renewcommand\dblfloatpagefraction{1}

\textwidth  .72\paperwidth	% WIDTH OF TEXT, REMAINS .28% FOR MARGINS
%
\setlength\@tempdima{.76\paperheight}	% HEIGHT OF TEXT WITH FOOTNOTES
\divide\@tempdima\baselineskip		% EXCLUDING HEAD (AND FOOT)
\@tempcnta=\@tempdima			% rounded to integer (#lines-1)
\setlength\textheight{\@tempcnta\baselineskip}
\addtolength\textheight{\topskip}

\voffset -1in
\topmargin   .05\paperheight	% FROM TOP OF PAGE TO TOP OF HEADING (0=1inch)
\headheight  .02\paperheight	% HEIGHT OF HEADING BOX.
\headsep     .03\paperheight	% VERT. SPACE BETWEEN HEAD AND TEXT.
\footskip    .07\paperheight	% FROM END OF TEX TO BASE OF FOOTER. (40pt)

\marginparsep 9\p@		% HOR. SPACE BETWEEN TEXT AND MARGINAL NOTE
\marginparpush 6\p@		% MIN. VERT. SPACE BETWEEN MARGINAL NOTES

\hoffset -1in				% TO ADJUST WITH PAPER:
\if@twoside				% IF TWO-SIDED:
	\oddsidemargin .13\paperwidth	% LEFT MARGIN FOR ODD PAGES (10)
	\evensidemargin .15\paperwidth	% LEFT MARGIN FOR EVEN PAGES (30)
	\marginparwidth .10\paperwidth	% TEXTWIDTH OF MARGINALNOTES
	\reversemarginpar		% BECAUSE OF TITLEPAGE.
\else					% IF ONE-SIDED:
	\oddsidemargin .14\paperwidth	% LEFT MARGIN FOR ODD PAGES (20)
	\evensidemargin .14\paperwidth	% LEFT MARGIN FOR EVEN PAGES (20)
	\marginparwidth .11\paperwidth	% TEXTWIDTH OF MARGINALNOTES
\fi					%
%%%%%%%%%%%%%%%%%%%%%%% HYPER (AND DRAFT) STUFF %%%%%%%%%%%%%%%%%%%%%%%
%\let\textref\@gobble
%\if@hyper			% IF NOHYPER WE DO LESS DAMAGE AS POSSIBLE.***
\ifpdf
      \input pdfcolor.tex
\else
\fi

\bgroup\catcode`\#=12\gdef\hash{#}\egroup	% DEFINED \hash=#.
%\fi
\def\H@tilde{\string~}
\newcommand{\href}[2]{\rule{0pt}{0pt}\bgroup\let~\H@tilde
		      \if@hyper\ifpdf
				    \def\hash{}%
				    \pdfstartlink attr{/Border [0 0 0]}
                                    user{/Subtype /Link /A << /S /URI /URI (#1) >>}%
					\pdfsetcolor{.9 .9 0 0}%
				\else
				    \noexpand\special{html:<A href="#1">}%
				\fi
		      \fi
		      {#2}\rule{0pt}{0pt}\egroup
		      \if@hyper\ifpdf
				    \Black\pdfendlink
			       \else
				    \special{html:</A>}%
			       \fi
                      \fi
		      }
% \intPlink was added because in pdflatex you need two different commands
% for internal and external links. For latex they are the same.
\newcommand{\intJlink}[2]{\rule{0pt}{0pt}\bgroup\let~\H@tilde
                        \if@hyper\ifpdf
                                       \def\hash{}%
                                       \pdfstartlink attr{/Border [0 0 0]}
                                          goto name{#1}%
                                       \pdfsetcolor{.9 .9 0 0}%
				  \else
                                       \noexpand\special{html:<A href="#1">}%
				  \fi
			\fi
                        {#2}\rule{0pt}{0pt}\egroup
                        \if@hyper\ifpdf
                                      \Black\pdfendlink
				 \else
                                      \special{html:</A>}%
                                 \fi
                        \fi
                        }


\newcommand{\name}[1]{\if@hyper\ifpdf
				    \pdfdest name{#1} fith%
			       \else
				    \noexpand\special% NAME HAS NO TAGGED TEXT HERE.
					{html:<A name="#1">}\special{html:</A>}%
			       \fi
		      \fi
		      }
\newcommand{\base}[1]{\if@hyper\ifpdf
                        \relax\JHEP@warn{Command base undefined for pdf output}
			%\pdfdest baseurl{#1} fith%
                       \else
                        \bgroup\let~\H@tilde
			\noexpand\special	% BASE HAS NO TAGGED TEXT.
			{html:<base href="#1">}\egroup
                       \fi\fi}
%------------------------------------------------------------------%
% SECTION TAGS and  THEIR REFERENCE IN TOC \d@t will be '.' for sections only
\if@hyper
\renewcommand{\@seccntformat}[1]{\name{sec\csname the#1\endcsname}%
				 \csname the#1\endcsname\d@t\hspace{1ex}}
\renewcommand{\numberline}[1]{\hb@xt@\@tempdima{\intJlink
			      {\hash\hyp@typ#1}{#1}\d@t\hfil}}
\else
\renewcommand{\@seccntformat}[1]{\csname the#1\endcsname\d@t\hspace{1ex}}
\renewcommand{\numberline}[1]{\hb@xt@\@tempdima{#1\d@t\hfil}}
\fi
%------------------------------------------------------------------%
% CITATION TAGS ARE TOGETHER WITH BIB STUFF.
% CITATION HREF
\def\@citex[#1]#2{%			% UNFORTUNATELY REDEFINED!!!!
  \let\@citea\@empty
  \@cite{\@for\@citeb:=#2\do
    {\@citea\def\@citea{,\penalty\@m\ }%
     \edef\@citeb{\expandafter\@firstofone\@citeb}%
     \if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}\fi
     \@ifundefined{b@\@citeb}{\mbox{\reset@font\bfseries ?}%
	\G@refundefinedtrue
	\@latex@warning
	  {Citation `\@citeb' on page \thepage \space undefined}}%
	{\edef\tmp@bn{\csname b@\@citeb\endcsname}%
	 \hbox{\intJlink{\hash bib\tmp@bn}{\tmp@bn}}}}}{#1}%		% **HYPER**
	 \if@draft\norm@note{CIT: }{#2}\fi			% **DRAFT**
	 }

%-----------------------------------------------------------------%
% LABEL, REF AND PAGEREF, TEXTREF, ~ COMPATIBLE:
\let\old@label\label						% OLD LATEX COMMAND.
\def\label{\bgroup\catcode`\>=15\catcode`\"=15 \@@label}		
\newcommand{\@@label}[1]{\egroup\name{ref-#1}%		% LABEL IN HYPER TAG.
			 \old@label{#1}%		% 
			 \if@draft%			% DRAFT:
			 \ifmmode\math@note{#1}%
			 \else\norm@note{}{LAB: #1}\fi%
			 \fi%
			 }
\if@hyper
\let\old@ref\ref \let\old@pageref\pageref		% OLD LATEX COMMANDS.
\renewcommand{\ref}[1]{\@ifundefined{r@#1}{}{\intJlink{\hash ref-#1}}%
		       {\old@ref{#1}}} % LABEL INSIDE HREF.
\renewcommand{\pageref}[1]{\@ifundefined{r@#1}{}{%	% UNDEFINED => NO HREF
	      \edef\tmp@ref{\noexpand\@secondoftwo\csname r@#1\endcsname}%
	      \intJlink{\hash pag\tmp@ref}}{\old@pageref{#1}}}
\fi
\newcommand{\textref}[2]{\@ifundefined{r@#1}
			{%
			\protect\G@refundefinedtrue
			\nfss@text{\reset@font\bfseries ?#2?}%
   			\@latex@warning{Reference `#1' on page \thepage \space
				             undefined}}
			{\vrule height \z@ width \z@\intJlink{\hash ref-#1}{#2}}}
%------------------------------------------------------------------%
%%%%%%%%%%%%%%%%%%%%%%%%%% END HYPER-STUFF %%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%% JHEP HEADINGS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\ps@JHEP{% 			
    \def\@oddfoot{\ifnum\thepage=0\ifnum\Jacce@year>2001\if@JHEP
		\Jcopyright@box\fi\hfill % copyright only on front page of published papers
		\if@Jspecialurl\unhbox\Jspecial@url\else\if@JHEP\unhbox\Jpaper@url\fi\fi\fi %possible url
		\else\reset@font\hfil-- \thepage\ --\hfil\fi} % page numbers on other pages
    \if@draft\edef\cur@opt{\@curroptions}\fi
    \def\@oddhead{\name{pag\thepage}\hfil\if@draft\copy\drft@box\fi}
    \if@proc
	\def\@oddhead{\name{pag\thepage}%
		      \smash{\if@draft\raise 2.5em\rlap{\copy\drft@box}\fi
		      	     \vbox{\hsize=\textwidth\noindent
			     \copy\conf@box\hfill
			     \copy\@firstaubox\vskip.17em \hrule}}%
		      }%
    \fi
    \if@twoside\let\@evenhead\@oddhead\let\@evenfoot\@oddfoot\fi
    \let\@mkboth\@gobbletwo
    \let\sectionmark\@gobble
    \let\subsectionmark\@gobble
    }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TITLE PAGE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\maketitle{\JHEP@ignol{\maketitle}}
\newcommand\auto@maketitle{\begingroup
    \renewcommand\thefootnote{\@fnsymbol\c@footnote}%
    \def\@makefnmark{\rlap{\@textsuperscript{\normalfont\@thefnmark}}}%
    \long\def\@makefntext##1{\parindent 1em\noindent
            \hb@xt@1.8em{\hss\@textsuperscript{\normalfont\@thefnmark}}##1}%
    \let\footnote\thanks%
	\newpage				%
	\if@proc				% IF PROCEEDINGS: 
	 \global\let\@nodocument\relax		% LaTeX FOULED:)
	\@maketitle				% 
	 \@thanks				% TITLE THANKS IN 1st COLUMN
	 \let\@evenfoot\@empty			% NO PAGENO.
 	 \let\@oddfoot\@empty
	 \setcounter{page}{1}%
	 \thispagestyle{empty}%			% PROCS HAVE NO PAGENUMBER
	\else
	 \@maketitle				% CALL ACTUAL FORMATTING
	 \@thanks				% TITLE THANKS
	 %\let\@evenfoot\@empty			% NO PAGENO.
 	 %\let\@oddfoot\@empty
	 \thispagestyle{JHEP} 
 	 \setcounter{page}\z@
	 \newpage				% FINE PAGINA
	\fi	
  \endgroup
  \setcounter{footnote}{0}%			
  \if@todotoc					% IF THERE IS A SECTION
      \noindent\rule\textwidth{.1pt}		% THEN MAKE TOC...
      \vskip 2em \@plus 3ex \@minus 3ex
      \tableofcontents
      \vskip 2em \@plus 3ex \@minus 3ex
      \noindent\rule\textwidth{.1pt}
      \vskip 2em \@plus 3ex \@minus 3ex
  \fi
  \if@preprint\else
  	\if@proc
	  \gdef\tableofcontents{\JHEP@igno{\tableofcontents\space there is no toc in proceedings}}
  	\else
	  \gdef\tableofcontents{\JHEP@igno{\tableofcontents\space is automatic}}
  	\fi
  \fi
  \global\let\thanks\@gobble
%  \setbox\@tmpbox=\vbox{\rm\@author}%		% FOR PROCS RESET HEADERS
%  \global\let\maketitle\relax			% NO LONGER EXISTS.
  \global\let\@maketitle\relax			%
  \global\let\@thanks\@empty			%
  \global\let\@author\@empty			% KILL ALL 
  \global\let\@date\@empty			%
  \global\let\@title\@empty			%
  \global\let\@abstract\@empty			%
  \global\let\title\relax			%
  \global\let\author\relax			%
  \global\let\date\relax			%
  \global\let\and\relax				%
  \global\let\email\@gobble
  \global\let\received\relax
  \global\let\revised\relax
  \global\let\accepted\relax
  \global\let\JHEPcopydate\relax
  \global\let\JHEPspecialurl\relax
  \global\let\keywords\relax
  \global\let\endkeywords\relax
}
%%%%%%%%%%%%%%%%%%%%%%%%%% ACTUAL TITLEPAGE %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newskip\titlesk@pa \newskip\titlesk@ja		% Skips for titlepage
\newskip\titlesk@pb \newskip\titlesk@jb		%
\newskip\titlesk@pc \newskip\titlesk@jc		%
\newskip\titlesk@pd				%
\titlesk@pa= 1.6em plus .4em%			% Before title (papers)
\titlesk@pb= 2em   plus .06em minus  .5ex%	% Between title/rule
\titlesk@pc= 2em   plus .05em minus 1.2ex%	% Before authors
\titlesk@pd= 2em   plus .06em minus  .5ex%	% After proc rule      	 
\titlesk@ja= 1.6em plus .4fil%			% Before title (proceedings)
\titlesk@jb= 2em   plus .06fil minus  .5ex%	% Between title/rule
\titlesk@jc= 2em   plus .05fil minus 1.2ex%	% Before authors

\def\@maketitle{%				% PAGE IS FLUSHED LEFT
\begin{flushleft}%				% PAY ATTENTION TO \par'S
%header for preprints
\if@preprint					%%% PREPRINT HEADER: 
\vskip-7em					%
\underline{\tiny Preprint typeset 		%
                 in JHEP style -		%
  		\if@hyper{HYPER VERSION}	%
		\else{PAPER VERSION}\fi } 	%
\normalsize\hfill%				% *** MAYBE PUT IN A ZERO BOX
\begin{tabular}[t]{r}\@preprint\end{tabular}% % PREPRINT NUMBERS
\else						%
  % header for proceedings
  \if@proc					%%% PROCEEDINGS: LOGO ETC..
    \vskip-4.48em\hfill\copy\conf@box
    \vskip-.7\baselineskip\logo\hrulefill
    \vskip-.4\baselineskip\hskip32\p@%	        % *** IDEM BOXIZE
		{\tiny PROCEEDINGS}
  \else
  % 					        %%% PUBLISHED: LOGO  ETC..
  %header for published (after 2001)
    \ifnum\Jacce@year>2001
       \vskip-7em\hfill
       {\small\scshape Published by Institute of Physics 
	               Publishing for SISSA/ISAS}
       \vskip-.7\baselineskip\logo\hrulefill
       \vskip-1.5\baselineskip\hskip21.73\p@%	% *** IDEM BOXIZE
       \hfill{\parbox[t]{30em}{\begin{flushright}\setlength\baselineskip{11pt}\footnotesize
				\Jrece@cs\\
				\if@revi\Jrevi@cs\\\fi
				\Jacce@cs
			      \end{flushright}}}%
    \else
    % header for published (december 2001)  *** TO BE REMOVED IN JHEP4...
    \vskip-7em\hfill{\small\Jrece@cs{\it,\ }\Jacce@cs
    \vskip-.7\baselineskip\logo\hrulefill
    \vskip-.5\baselineskip\hskip23\p@%	% *** IDEM BOXIZE
 		{\tiny \if@hyper{HYPER VERSION}\else{PAPER VERSION}\fi}
    \if@revi\hfill\Jrevi@cs\fi}

    \fi
  \fi
\fi\null
% end headers
% title page: skips are different for procs (p) and jhep or preprints (j)
% see above
  \if@proc
   \vskip \titlesk@pa
  \else
   \vskip \titlesk@ja		   % vspace before title
  \fi
% TITLE 
  {\LARGE \sffamily                
        \bfseries                  
        \@title\par}%                large sans-serif bf
  \if@proc
    \vskip \titlesk@pb             
  \else
    \vskip \titlesk@jb             % vspace between title and rule
  \fi
  \if@proc
% RULE
    \hrule height \p@%               for proc = 1pt
  \else
    \hrule height 1.5\p@%            otherwise = 1.5pt.
  \fi
  \if@proc
    \vskip \titlesk@pb             
  \else
    \vskip \titlesk@jb		   % vspace between rule and authors
  \fi
% AUTHORS\\ADDRESSES
  \vskip-\auth@skip
  {\normalsize \bfseries \sffamily
	\@author \par}                            
  \if@proc
    \vskip \titlesk@pc
  \else
    \vskip \titlesk@jc             % vspace between authors and abstract
  \fi
% ABSTRACT IF PRESENT (SHOULD)
  \if@proc
    \centerline{\parbox{.9\textwidth}%	% narrower abstract for proceedings
		    {\abstract@cs}}%
  \else
    \parbox\textwidth{\abstract@cs}%	
  \fi
  \normalsize
% KEYWORDS IF PRESENT
  \if@keywords	
    \if@proc
	\vskip \titlesk@pc	   
    \else
	\vskip .9\titlesk@jc	   % vspace between abstract and keywords
    \fi
    \par
    \@keywords				
  \fi
% DEDICATION, IF PRESENT
  \dedic@box				
% RULE (only for procs)
  \if@proc
    \vskip \titlesk@pb
    \hrule height 1\p@
    \vskip \titlesk@pd
  \fi
\end{flushleft}%			% FINISHED.
}
%%%%%%%%%%%%%%%%%%%%%%%%%%% STANDARD STUFF %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setcounter{secnumdepth}{3}
\newcounter {part}
\newcounter {section}
\newcounter {subsection}[section]
\newcounter {subsubsection}[subsection]
\newcounter {paragraph}[subsubsection]
\newcounter {subparagraph}[paragraph]
\renewcommand\thepart         {\@Roman\c@part}
\renewcommand\thesection      {\@arabic\c@section}
\renewcommand\thesubsection   {\thesection.\@arabic\c@subsection}
\renewcommand\thesubsubsection{\thesubsection.\@arabic\c@subsubsection}
\renewcommand\theparagraph    {\thesubsubsection.\@arabic\c@paragraph}
\renewcommand\thesubparagraph {\theparagraph.\@arabic\c@subparagraph}
%%%%%%%%%%%%%%%%%%%%%%%%%%% SECTION FORMATS %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\secstyle{\bfseries}
\def\ts@flag{\let\d@t.%					% Sections get ``.''
	     \immediate\write\@auxout			% IF THERE IS A SECTION
	     {\string\global\string\@todotoctrue}}	% THEN SIGNAL IN AUX.

\newcommand\part{\par
   \addvspace{4ex}%
   \@afterindentfalse
   \secdef\@part\@spart}

\def\@part[#1]#2{\ts@flag
    \ifnum \c@secnumdepth >\m@ne
      \refstepcounter{part}%			% DAMN LATEX !!! BELOW,
      \addcontentsline{toc}{part}{\string\intJlink	% UNFORTUNATELY, NO NUMBERLINE:
				  {\string\hash\space part\the\c@part}%
				  {\thepart}\hspace{1em}#1}%
    \else
      \addcontentsline{toc}{part}{#1}%
    \fi
    {\parindent \z@ \raggedright
     \interlinepenalty \@M
     \normalfont
     \ifnum \c@secnumdepth >\m@ne
       \name{part\the\c@part}\Large\bfseries \partname~\thepart
       \par\nobreak
     \fi
     \huge \bfseries #2%
     \markboth{}{}\par}%
    \nobreak
    \vskip 3ex
    \@afterheading\let\d@t\relax}
\def\@spart#1{%
    {\parindent \z@ \raggedright
     \interlinepenalty \@M
     \normalfont
     \huge \bfseries #1\par}%
     \nobreak
     \vskip 3ex
     \@afterheading}

\newcommand\section{\@startsection{section}{1}{\z@}%
                                   {-3.5ex \@plus -1.3ex \@minus -.7ex}%
                                   {2.3ex \@plus.4ex \@minus .4ex}%
                                   {\normalfont\large\secstyle}}
\newcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                   {-2.3ex\@plus -1ex \@minus -.5ex}%
                                   {1.2ex \@plus .3ex \@minus .3ex}%
                                   {\normalfont\normalsize\secstyle}}
\newcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                   {-2.3ex\@plus -1ex \@minus -.5ex}%
                                   {1ex \@plus .2ex \@minus .2ex}%
                                   {\normalfont\normalsize\secstyle}}
\newcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                                   {1.75ex \@plus1ex \@minus.2ex}%
                                   {-1em}%
                                   {\normalfont\normalsize\bfseries}}
\newcommand\subparagraph{\@startsection{subparagraph}{5}{\parindent}%
                                   {1.75ex \@plus1ex \@minus .2ex}%
                                   {-1em}%
                                   {\normalfont\normalsize\bfseries}}

% ---- turnaround for sections with figures ------ %
\def\bef@sec{\iffigprocessing\JHEP@warnl{Floating figure \the\ffigcount\space
						and startsection colliding}\fi
	     \iftabprocessing\JHEP@warnl{Floating table \the\ftabcount\space
						and startsection colliding}\fi
	     \edef\bef@everypar{\the\everypar}}	% HACK FOR FLOATS AND \everypar
\def\aft@sec{\let\d@t\relax			% RESTORE: NO DOTTED SUBSECS..
	     \edef\tmp@everypar{\the\everypar}% % DELETED CLUBPENALTY, BELOW.
	     \everypar\expandafter{\bef@everypar{\tmp@everypar}}}% RESTORE.
\let\old@sec\section				%
\let\old@ssec\subsection			%
\let\old@sssec\subsubsection			% OLD SECTIONING COMMANDS.
\let\old@par\paragraph				%
\let\old@spar\subparagraph			%
% ------- new forms ------- %
\renewcommand{\section}{\secdef\JHEP@sec\JHEP@secs}
\renewcommand{\subsection}{\secdef\JHEP@ssec\JHEP@ssecs}
\renewcommand{\subsubsection}{\secdef\JHEP@sssec\JHEP@sssecs}
\renewcommand{\paragraph}{\secdef\JHEP@par\JHEP@pars}
\renewcommand{\subparagraph}{\secdef\JHEP@spar\JHEP@spars}
% ---- unstarred forms ---- %
\def\JHEP@sec[#1]#2{\ts@flag\bef@sec\old@sec[#1]{#2}\aft@sec}
\def\JHEP@ssec[#1]#2{\bef@sec\old@ssec[#1]{#2}\aft@sec}
\def\JHEP@sssec[#1]#2{\bef@sec\old@sssec[#1]{#2}\aft@sec}
\def\JHEP@par[#1]#2{\bef@sec\old@par[#1]{#2}\aft@sec}
\def\JHEP@spar[#1]#2{\bef@sec\old@spar[#1]{#2}\aft@sec}
% ----- starred forms ----- %
\def\JHEP@secs#1{\bef@sec\old@sec*{#1}\aft@sec}
\def\JHEP@ssecs#1{\bef@sec\old@ssec*{#1}\aft@sec}
\def\JHEP@sssecs#1{\bef@sec\old@sssec*{#1}\aft@sec}
\def\JHEP@pars#1{\bef@sec\old@par*{#1}\aft@sec}
\def\JHEP@spars#1{\bef@sec\old@spar*{#1}\aft@sec}
% ----- end hack for sections with floats --------%

\if@twocolumn
  \setlength\leftmargini  {2em}
\else
  \setlength\leftmargini  {2.5em}
\fi
\leftmargin  \leftmargini
\setlength\leftmarginii  {2.2em}
\setlength\leftmarginiii {1.87em}
\setlength\leftmarginiv  {1.7em}
  \setlength\leftmarginv  {1em}
  \setlength\leftmarginvi {1em}
\setlength  \labelsep  {.5em}
\setlength  \labelwidth{\leftmargini}
\addtolength\labelwidth{-\labelsep}
\@beginparpenalty -\@lowpenalty
\@endparpenalty   -\@lowpenalty
\@itempenalty     -\@lowpenalty
\renewcommand\theenumi{\@arabic\c@enumi}
\renewcommand\theenumii{\@alph\c@enumii}
\renewcommand\theenumiii{\@roman\c@enumiii}
\renewcommand\theenumiv{\@Alph\c@enumiv}
\newcommand\labelenumi{\theenumi.}
\newcommand\labelenumii{(\theenumii)}
\newcommand\labelenumiii{\theenumiii.}
\newcommand\labelenumiv{\theenumiv.}
\renewcommand\p@enumii{\theenumi}
\renewcommand\p@enumiii{\theenumi(\theenumii)}
\renewcommand\p@enumiv{\p@enumiii\theenumiii}
\newcommand\labelitemi{$\m@th\bullet$}
\newcommand\labelitemii{\normalfont\bfseries --}
\newcommand\labelitemiii{$\m@th\ast$}
\newcommand\labelitemiv{$\m@th\cdot$}
\newenvironment{description}
               {\list{}{\labelwidth\z@ \itemindent-\leftmargin
                        \let\makelabel\descriptionlabel}}
               {\endlist}
\newcommand*\descriptionlabel[1]{\hspace\labelsep
                                \normalfont\bfseries #1}
%%%%%%%%%%%%%%%%%%%%%%%%%% AUTHORS/ADDRESSES %%%%%%%%%%%%%%%%%%%%%%%%%%
% *** After proceedings, the authors go in a hbox. => \break does not work!!
% *** if no address nobody closes the box!
\newif\if@speaker\@speakerfalse
\newif\if@dblspeak\@dblspeakfalse
\newtoks\prev@t
\newtoks\cur@t
\newbox\@firstaubox
\newskip\addr@skip\addr@skip=\if@proc .6em\@plus.02em\@minus.3ex
			     \else .6em\@plus.02fil\@minus.3ex \fi
\newskip\auth@skip\auth@skip=\if@proc .6em\@plus.03em\@minus.2ex
			     \else .6em\@plus.03fil\@minus.2ex \fi
\renewcommand\@author{\parskip\z@
%		      \def\@noaddr{\setbox\@tmpbox\vbox\bgroup\let\\\par}%
		      \def\\{\egroup			% CLOSE & aftergroup!
			\par				% FIRST TIME \\=>ADDR.
			\vskip\addr@skip		% GLUE UNDER AUTHOR
			\hskip1em%			% ADDRESS INDENT
			\vbox\bgroup\hsize=.9\textwidth	% 
			\small\it\raggedright		% STYLE FOR ADDRESSES
			\def\\{\par\leavevmode\ignorespaces}%\let\\\relax%
			\leavevmode\ignorespaces}%
			}
\renewcommand\author[1]{%
		\global\@authortrue			%
		\prev@t=\expandafter{\@author}%		% TWO TOKEN LISTS.
		\cur@t={\vskip\auth@skip		% glue before auth.
			\vtop\bgroup #1\egroup		% ACTUAL AUTH.\\ADD.
			\par}%				%
		\long\xdef\@author{\the\prev@t\the\cur@t}%STORE ALL IN \@AUTHOR
		}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% SPEAKER %%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\speaker[1]{\if@speaker\global\@dblspeaktrue\fi
			\global\@speakertrue
			\global\setbox\@firstaubox
			\hbox{\let\thanks\@gobble
				\let\footnote\@gobble 
				\rm #1}%
			#1\thanks{Speaker.}\
			}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CONFERENCE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newbox\conf@box
\newcommand\conference[1]{\global\setbox\conf@box\hbox{%
			 \itshape #1}\@conftrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RECEIVED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\received[1]{\gdef\Jrece@cs{{\scshape\receivedname} 
                                       {\itshape #1}}\@recetrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% REVISED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\revised[1]{\gdef\Jrevi@cs{{\scshape\revisedname}
                                      {\itshape #1}}\@revitrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PUBLISHED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\accepted[1]{\gdef\Jacce@cs{{\scshape\acceptedname}
                                       {\itshape #1}}\@accetrue}
%%%%%%%%%%%%%%%%%%%%%%%%%% COPYRIGHT DATE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newbox\Jcopy@date
\newcommand\JHEPcopydate[1]{\global\setbox\Jcopy@date
                        \hbox{\scriptsize #1}\global\@Jcopytrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DEDICATED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\dedic@box{\relax}
\newcommand\dedicated[1]{\gdef\dedic@box{\vskip2em minus 1.2ex
                              \vbox{\small\it\raggedleft #1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%% ACKNOWELEDGMENTS %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\acknowledgments{\section*{\acknowlname}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% EMAIL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\email[1]{{\tt\href{mailto:#1}{#1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PREPRINT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\@preprint\relax
\newcommand\preprint[1]{\long\gdef\@preprint{#1}} 
%%%%%%%%%%%%%%%%% SPECIAL URL overrides paper@url %%%%%%%%%%%%%%%%%%%%%
\newbox\Jspecial@url
\newcommand\JHEPspecialurl[1]{\global\setbox\Jspecial@url\hbox{\tiny\ttfamily
			#1}\@Jspecialurltrue}
%%%%%%%%%%%%%%%%%%%%%%%%% FILE NAME AND URL %%%%%%%%%%%%%%%%%%%%%%%%%%%
\global\newbox\Jacce@month
\global\newcount\Jacce@year
\global\newbox\Jacce@number
\def\Jsplit@ident#1(#2)#3.{\global\setbox\Jacce@month\hbox{\tiny\ttfamily #1}
			  \global\Jacce@year= #2
			  \global\setbox\Jacce@number\hbox{\tiny\ttfamily #3}

\newbox\Jpaper@url
\gdef\Jfile@name{\hbox{\tiny\ttfamily
		jhep\unhcopy\Jacce@month\the\Jacce@year\unhcopy\Jacce@number}}

\global\setbox\Jpaper@url\hbox{\tiny\ttfamily 
		http://jhep.sissa.it/archive/papers/\Jfile@name/\Jfile@name.pdf}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COPYRIGHT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\Jcopyright@box{\hbox{\if@preprint\else{\scriptsize $\copyright$
		SISSA/ISAS\ \if@Jcopy\unhbox\Jcopy@date\else\the\year\fi}\fi}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ABSTRACT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% *** For beton! We need a cs, not a box. Maybe also for refs.. %%%%%%

\newcommand{\abstract}[1]%		% ABSTR. IN NORMALSIZE
	{\gdef\abstract@cs{		% cs FOR WHOLE ABSTRACT
	{\if@proc\small\else\fi
	\noindent{\scshape\abstractname}\ \ignorespaces #1}}
	\normalsize
	\global\@abstracttrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% KEYWORDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@keywords{\relax}%                   % CS FOR WHOLE KEYWORDS
\def\keywords{\bgroup\gdef\@comma{,}\catcode`\ =\active\catcode`,=\active
		\@@keywords}
\begingroup
\catcode`\ =\active\catcode`,=\active\global
\def\@@keywords#1{\gdef\@keywords{\noindent{\scshape\keywordsname}
		\bgroup\def, {+}\def {_}%	%ATTENTION: NO EXPANSION.
		\href{http://jhep.sissa.it/stdsearch}%
						{\let,\@comma\let \ #1}.
		\egroup}\egroup\global\@keywordstrue}%
\endgroup
%%%%%%%%%%%%%%%%%%%%%%%%%% OTHER ENVIRONMENTS %%%%%%%%%%%%%%%%%%%%%%%%%
\newenvironment{verse}
               {\let\\\@centercr
                \list{}{\itemsep      \z@
                        \itemindent   -1.5em%
                        \listparindent\itemindent
                        \rightmargin  \leftmargin
                        \advance\leftmargin 1.5em}%
                \item\relax}
               {\endlist}
\newenvironment{quotation}
               {\list{}{\listparindent 1.5em%
                        \itemindent    \listparindent
                        \rightmargin   \leftmargin
                        \parsep        \z@ \@plus\p@}%
                \item\relax}
               {\endlist}
\newenvironment{quote}
               {\list{}{\rightmargin\leftmargin}%
                \item\relax}
               {\endlist}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THEOREMS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if@twothms\@twothmsfalse

\if@preprint%\ifx\@thmcountersep\@undefined
%\def\@xthm#1#2{\@begintheorem{#2}{\csname the#1\endcsname.}\ignorespaces}% after thm number
\else									 % if published or proc
\def\@xthm#1#2{\@begintheorem{#2\if@twothms\else.\fi}			 % theorems are numbered
		{\if@twothms\csname the#1\endcsname.\fi}		 % only if more than one
		\ifnum \csname the#1\endcsname>1 \immediate\write\@auxout% and not within sections
				{\string\global\string\@twothmstrue}\fi
		\ignorespaces}
\fi

\newcommand\Proof{\noindent\emph{Proof.}\ }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\appendix{\par
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \renewcommand\thesection{\@Alph\c@section}}

%%%%%%%%%%%%%%%%%%%%%%%%%%% SOME MORE LENGHTS %%%%%%%%%%%%%%%%%%%%%%%%%
\setlength\arraycolsep{2\p@}		% TO MATCH eqnarrays<->equations
\setlength\tabcolsep{6\p@}
\setlength\arrayrulewidth{.4\p@}
\setlength\doublerulesep{2\p@}
\setlength\tabbingsep{\labelsep}
\skip\@mpfootins = \skip\footins
\setlength\fboxsep{3\p@}
\setlength\fboxrule{.4\p@}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THE EQUATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\theequation{\ifnum\c@section=0\else\thesection.\fi
			  \@arabic\c@equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% FIGURES, TABLES %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcounter{figure}
\renewcommand\thefigure{\@arabic\c@figure}
\def\fps@figure{Htbp}
\def\ftype@figure{1}
\def\ext@figure{lof}
\def\fnum@figure{\figurename~\thefigure}
\newenvironment{figure}
               {\@ENVwarn{\FIGURE{...}}\@float{figure}}
               {\end@float}
\newenvironment{figure*}
               {\@ENVwarn{\FIGURE{...}}\@dblfloat{figure}}
               {\end@dblfloat}
\newcounter{table}
\renewcommand\thetable{\@arabic\c@table}
\def\fps@table{tbp}
\def\ftype@table{2}
\def\ext@table{lot}
\def\fnum@table{\tablename~\thetable}
\newenvironment{table}
               {\@ENVwarn{\TABLE{...}}\@float{table}}
               {\end@float}
\newenvironment{table*}
               {\@ENVwarn{\TABLE{...}}\@dblfloat{table}}
               {\end@dblfloat}
%%-----------------------------------------------------------------%%
\newcommand{\FIGURE}[2][v]{\begin{floatingfigure}[#1]#2
                                        \end{floatingfigure}}
\newcommand{\TABLE}[2][v]{\begin{floatingtable}[#1]{#2}
                                        \end{floatingtable}}
\newcommand{\EPSFIGURE}[3][v]{\begin{floatingfigure}[#1]\epsfig{file=#2}
                                        \caption{#3}\end{floatingfigure}}
\newcommand{\TABULAR}[4][v]{\begin{floatingtable}[#1]{\begin{tabular}{#2}
					#3\end{tabular}}\caption{#4}
                                        \end{floatingtable}}
%Check below, and put automatic width ***
\newcommand{\DOUBLEFIGURE}[5][ht]{\@dblfloat{figure}[#1]\centerline{%
		\parbox{.45\textwidth}{\centerline{\epsfig{file=#2}}}~~~~
		\parbox{.45\textwidth}{\centerline{\epsfig{file=#3}}}}
		\centerline{\parbox[t]{.45\textwidth}{\caption{#4}}~~~~
		\parbox[t]{.45\textwidth}{\caption{#5}}}\end@dblfloat}
\newcommand{\DOUBLETABLE}[5][ht]{\@dblfloat{table}[#1]\centerline{%
		\parbox{.45\textwidth}{\centerline{#2}}~~~~
		\parbox{.45\textwidth}{\centerline{#3}}}
		\centerline{\parbox[t]{.45\textwidth}{\caption{#4}}~~~~
		\parbox[t]{.45\textwidth}{\caption{#5}}}\end@dblfloat}
%%%%%%---------------- FROM FLOATFLT PACKAGE ------------------%%%%%%%%
%% Original file `floatflt.sty', modified by F.Nesti <nesti@sissa.it> to:
%% be inserted in JHEP.cls;
%% correct float placement when shifting past pages;
%% correct incompatibility with \marginpar;
%% correct incompatibility with \@startsection;
%% correct persisting indentation in following pars;
%% let float also at beginning of pages; 
%% avoid the widht specification.
%% 
%% Original was 1994-1996 by Mats Dahlgren <matsd@physchem.kth.se>. 
%% 
%%%%%%%%\NeedsTeXFormat{LaTeX2e}[1994/06/01]		%LEFT THIS STUFF TO 
%%%%%%%%\ProvidesPackage{floatflt}[1996/02/27 v. 1.3]	%RECONVERT TO PACKAGE.
\newcounter{OptionTest}
\if@twoside
 \setcounter{OptionTest}{0}
\else							% POS: 2side=p/1side=r
 \setcounter{OptionTest}{1}
\fi
%%%%%%%%\DeclareOption{rflt}{\setcounter{OptionTest}{1}}
%%%%%%%%\DeclareOption{lflt}{\setcounter{OptionTest}{2}} % CHOSEN.
%%%%%%%%\DeclareOption{vflt}{\setcounter{OptionTest}{0}}
%%%%%%%%\DeclareOption*{\OptionNotUsed}
%%%%%%%%\ProcessOptions
\newbox\@tmpbox
\newbox\figbox
\newbox\tabbox
\newbox\pagebox
\newcount\ffigcount
\newcount\ftabcount
\newcount\hangcount
\newcount\nosuccesstryfig
\newcount\nosuccesstrytab
\newdimen\figgutter   \figgutter=1truepc
\newdimen\tabgutter   \tabgutter=1truepc
\newdimen\fl@wd
\newdimen\fl@ht
%\newdimen\fl@gut
\newdimen\htdone      \htdone=\z@
\newdimen\pageht
\newdimen\startpageht
\newdimen\floatfltwidth
\newdimen\fltitemwidth
\newif\iftryingfig     \tryingfigfalse
\newif\iftryingtab     \tryingtabfalse
\newif\ifdoingfig      \doingfigfalse
\newif\ifdoingtab      \doingtabfalse
\newif\iffigprocessing \figprocessingfalse
\newif\iftabprocessing \tabprocessingfalse
\newif\ifpageafterfig  \pageafterfigfalse
\newif\ifpageaftertab  \pageaftertabfalse
\newif\ifoddpages
\newif\ifoutput
\newtoks\outputpretest
\def\@captype{}
%%---------------- ORRIBLE HACKS, SORRY -------------------------%%
\let\old@marginpar\marginpar				% 
\renewcommand\marginpar[1]{{\outputpretest={\outputtrue}% REDEF \marginpar.
			    \old@marginpar{#1}}}	%
\def\g@addto#1#2{{\toks@\expandafter{#1#2}%
		  \xdef#1{\the\toks@}}}%
\def\postpone@captions{%			%
%	\global\let\tmp@label\label		% REDEF \caption AND 
	\global\let\tmp@caption\caption		% \label, LATER.
	\global\let\later@capt\relax		% UN PO' PESANTI 
	\gdef\later@label{}%			% MA D'ALTRONDE...
	\let\J@ref\ref\def\ref{\protect\J@ref}% % protect ref in captions.. 
	\renewcommand\caption{\@ifnextchar[\J@@caption\J@caption}%
	\newcommand\J@caption[1]{\gdef\later@capt{\tmp@caption{##1}}}% LOCAL!!
	\newcommand\J@@caption[2][v]%
				{\gdef\later@capt{\tmp@caption[##1]{##2}}}% LOCAL!!
	\renewcommand\@@label[1]{\egroup\name{ref-##1}%	% TAG WHERE CALLED, AT LEAST,
			       \if@draft\norm@note{}{LAB: ##1}\fi% & DRAFTNOTE.
			       \g@addto\later@label{\old@label{##1}}}%
			}
\AtEndDocument{\iftryingfig\JHEP@warnl{Floating figure \the\ffigcount\space
					remains undone}\fi
		\iftryingtab\JHEP@warnl{Floating table \the\ftabcount\space
					remains undone}\fi
		\if@JHEP\ifnum\Jacce@year>2001\if@Jcopy\else
		\ifnum\the\Jacce@year=\the\year\else
		\JHEP@warnl{The acceptance date
		\the\Jacce@year\space is different from today's
		\the\year}\fi\fi\fi\fi} % the copyright date must be that
			  %  of publication if it differs from the one in the
		 	  % identifier it can be forced using command \JHEPcopydate
%%----------------- FIGURE ---------------------------------------%%
\newenvironment{floatingfigure}[1][v]%
{\@tfor \@tempa :=#1\do {\xdef\@fside{\@tempa}}%
 \global\advance\ffigcount by 1%
 \iffigprocessing {\count0=\ffigcount\advance\count0 by -1%
   		   \JHEP@warnl{Floating figures \the\count0\space\space and
       			\the\ffigcount\space colliding}}\fi
 \iftabprocessing  \JHEP@warnl{Floating table \the\ftabcount\space and 
			floating figure \the\ffigcount\space colliding}\fi
 \postpone@captions
 \global\setbox\@tmpbox=\hbox\bgroup% begin of figbox %HBOX FOR AUTO WIDTH!
}
{%
\egroup%				% CALCULATE WIDTH (NO CAPTION FOR NOW)
\global\setlength{\floatfltwidth}{\the\wd\@tmpbox}%
% New behavior:	wd < .6 columnwidth => floatflt.
%		wd < columnwidth    => float{figure}
%		wd > columnwidth    => dblfloat{figure}
\ifdim\floatfltwidth<.6\columnwidth%	% IF NOT TOO WIDE OK:
 \global\setbox\figbox=\vbox{\hsize=\floatfltwidth
			     \def\@captype{figure}%
			     \noindent\unhbox\@tmpbox
			     \later@capt\later@label}%
 \global\figprocessingtrue
 \global\everypar={\tryfig\oldeverypar}% must be set globally!
 \figinsert\par
\else%					% ELSE NORMAL LATEX FIGURE, SIGH.
% \JHEP@mess{Floating figure \the\ffigcount\space is 
%			wide becomes a LaTeX float}%
 \if\@fside v \def\@fside{ht}\fi
 \ifdim\floatfltwidth<\columnwidth
    \def\@@tempa{\@float{figure}[}\let\@@tempb\end@float
 \else
    \def\@@tempa{\@dblfloat{figure}[}\let\@@tempb\end@dblfloat
 \fi
 \expandafter\@@tempa\@fside]\center\unhbox\@tmpbox\later@capt\later@label\@@tempb
\fi
}
%%------------ TABLE ----------------------------------------------%%
\newenvironment{floatingtable}[1][v]%
{\@tfor \@tempa :=#1\do {\global\edef\@tside{\@tempa}}%
 \global\advance\ftabcount by 1%
 \iftabprocessing {\count0=\ftabcount\advance\count0 by -1%
     		   \JHEP@warnl{Floating tables \the\count0\space
            		\space and \the\ftabcount \space colliding}}\fi
 \iffigprocessing  \JHEP@warnl{Floating figure \the\ffigcount\space and 
			floating table \the\ftabcount\space colliding}\fi
 \postpone@captions
 \global\setbox\@tmpbox=\hbox\bgroup% begin of tabbox, ACTUALLY AN HBOX.
}
{%
\egroup% end of \tabbox, 		% ACTUALLY \@tmpbox
\global\setlength{\floatfltwidth}{\the\wd\@tmpbox}%
\ifdim\floatfltwidth<.6\columnwidth%	% IF NOT TOO WIDE OK:
  \global\setbox\tabbox=\vbox{\hsize=\floatfltwidth
			     \def\@captype{table}%
			     \noindent\unhbox\@tmpbox
			     \later@capt\later@label}%
  \global\tabprocessingtrue
  \global\everypar={\trytab\oldeverypar}%
  \tabinsert\par%
\else%					% ELSE NORMAL LATEX TABLE.
%  \JHEP@mess{Floating table \the\ftabcount\space is 
%			wide becomes a LaTeX float}%
  \ifdim\floatfltwidth<1.1\columnwidth
    \if\@tside v \def\@tside{ht}\fi
    \def\@@tempa{\@float{table}[}\let\@@tempb\end@float
  \else
    \if\@tside v \def\@tside{t}\fi
    \def\@@tempa{\@dblfloat{table}[}\let\@@tempb\end@dblfloat
  \fi
  \expandafter\@@tempa\@tside]%		% ACTUALLY CALL THE LATEX FLOAT
  \center\unhbox\@tmpbox\later@capt\later@label
  \@@tempb
\fi%
}
%----------- prepare for tries ----------------------------%
\def\figinsert{%
   \global\nosuccesstryfig=0%
   \global\outputpretest={\do@test}%
   \global\tryingfigtrue \global\doingfigfalse%
   \global\pageafterfigfalse}%
\def\tabinsert{%
   \global\nosuccesstrytab=0%
   \global\outputpretest={\do@test}%
   \global\tryingtabtrue \global\doingtabfalse%
   \global\pageaftertabfalse}%
%----------- init -----------------------------------------%
\AtBeginDocument{%
 \edef\oldoutput{\the\output}
 \output={\the\outputpretest\ifoutput\oldoutput\fi}%
 \outputpretest={\outputtrue}%
 \edef\oldeverypar{\the\everypar}% PERCHE' NESSUNO LO RIMETTE PIU' A POSTO?***
}
%---- tests during \outputpretest -------------------------%
\def\do@test{%
   \ifnum\outputpenalty=-10005
%	\output
     \setbox\pagebox=\vbox{\unvbox255}%
     \global\pageht=\ht\pagebox
     \global\outputfalse
     \unvbox\pagebox
     \dimen0=\pageht\advance\dimen0 by 2 \baselineskip
     \ifdim\dimen0>\vsize\pagebreak[4]\global\pageht\z@\fi
   \else
     \global\outputtrue
     \ifnum\outputpenalty>-\@Mi			%ie \marginpar's give penalty.
	\ifdoingtab\global\pageaftertabtrue\fi
	\ifdoingfig\global\pageafterfigtrue\fi
     \fi
   \fi}%
%-------- check for side ----------------------------------%
\def\chk@side#1{% DEFINED \fl@sid, BUT IF CHOSEN A DEFAULT, ELIMINATE ALL ***
	{\edef\fl@sid{#1}%
	  \if\fl@sid r\global\oddpagestrue\fi
          \if\fl@sid l\global\oddpagesfalse\fi
          \if\fl@sid p%
              \ifodd\c@page\global\oddpagesfalse
                \else\global\oddpagestrue\fi
          \fi
          \if\fl@sid v%
             \ifnum\theOptionTest=0%
                 \ifodd\c@page\global\oddpagesfalse
                   \else\global\oddpagestrue\fi
             \else
                  \ifodd\theOptionTest\global\oddpagestrue
                    \else\global\oddpagesfalse\fi
             \fi
          \fi
         }}%
%-------- get point in page -------------------------------%
\def\get@pageht{{\everypar={\relax}\setbox0=\lastbox
       		\parindent=\wd0 \parskip=\z@ \par
         	\penalty-10005 \leavevmode}}%
%-------- try at everypar ---------------------------------%
\def\tryfig{%
	\global\fl@ht\ht\figbox
	\global\fl@wd\wd\figbox
	\global\let\fl@gut\figgutter
      \iftryingfig
	\get@pageht
	\dimen0=\vsize
	\advance\dimen0 by -\pageht
	\advance\dimen0 by -2\baselineskip
	\ifdim\dimen0>\fl@ht
	  \chk@side\@fside
	  \dimen0=0.3\baselineskip
	  \vrule depth \dimen0 width \z@%height 1.5\baselineskip
	  \vadjust{\kern -\dimen0
	  \vtop to \dimen0{%
             \baselineskip=\dimen0
             \vss \vbox to 1ex{%
             \ifoddpages
               \hb@xt@\hsize{\hss\copy\figbox}%
             \else% leftsetting
               \hb@xt@\hsize{\copy\figbox\hss}%
             \fi
             \vss}\null}}%
	  \global\tryingfigfalse
	  \global\doingfigtrue
	  \global\startpageht=\pageht
	  \global\htdone=\z@
	  \dohang
	  \ifnum\nosuccesstryfig>0%
	   \JHEP@mess{Flt. fig. \the\ffigcount\space set on page \the\count0, 
	 		shifted \the\nosuccesstryfig\space par(s) forward}%
%	  \else
%	   \JHEP@mess{Floating figure \the\ffigcount\space 
%			set on page \the\count0}%
	  \fi
	\else
          \global\advance\nosuccesstryfig by 1
	\fi
      \else%				% IF NOT TRYING
	\ifdoingfig
	  \get@pageht
	  \global\htdone=\pageht
	  \global\advance\htdone by -\startpageht
	  \ifpageafterfig
	    \global\doingfigfalse% IN CASE A PAGEBREAK JUST BELOW?
	  \else
	    \dimen0=\fl@ht
	    \advance\dimen0 by .85\baselineskip	% .85 ENOUGH: WE ARE AT NEW PAR
%	    \typeout{FLOAT HT: \the\dimen0, HTDONE: \the\htdone}
	    \ifdim\htdone<\dimen0%
		\dohang
	    \else
		\global\doingfigfalse
	    \fi
	  \fi
	  \ifdoingfig\else\global\figprocessingfalse\fi% IF NO MORE DOING.
	\else
	  \global\outputpretest={\outputtrue}% NOT RESTORE EVPAR IF NOT DOING?
	\fi%			% END IF DOING
      \fi%			% END IF TRYING
}
\def\trytab{%
	\global\fl@ht\ht\tabbox
	\global\fl@wd\wd\tabbox
	\global\let\fl@gut\tabgutter
       \iftryingtab
	\get@pageht
       \dimen0=\vsize
       \advance\dimen0 by -\pageht
       \advance\dimen0 by -2\baselineskip
       \ifdim\dimen0>\fl@ht
	 \chk@side\@tside
         \dimen0=0.3\baselineskip
         \vrule depth \dimen0 width \z@
         \vadjust{\kern -\dimen0
         \vtop to \dimen0{%
             \baselineskip=\dimen0
             \vss \vbox to 1ex{%
             \ifoddpages
               \hb@xt@\hsize{\hss\copy\tabbox}%
             \else% leftsetting
               \hb@xt@\hsize{\copy\tabbox\hss}%
             \fi
             \vss}\null}}%
       \global\tryingtabfalse
       \global\doingtabtrue
       \global\startpageht=\pageht
       \global\htdone=\z@
       \dohang
       \ifnum\nosuccesstrytab>0%
	\JHEP@mess{Flt. tab. \the\ftabcount\space set on page \the\count0, 
			shifted \the\nosuccesstrytab\space par(s) forward}%
%       \else
%	\JHEP@mess{Floating table \the\ftabcount\space 
%			set on page \the\count0}%
       \fi
     \else
       \global\advance\nosuccesstrytab by 1
     \fi
     \else
     \ifdoingtab
       \get@pageht
    \global\htdone=\pageht
    \global\advance\htdone by -\startpageht
    \ifpageaftertab
      \global\doingtabfalse
    \else
      \dimen0=\fl@ht
      \advance\dimen0 by .85\baselineskip	% .85 ENOUGH: WE ARE AT NEW PAR
      \ifdim\htdone<\dimen0%
         \dohang
      \else
         \global\doingtabfalse
      \fi
    \fi
    \ifdoingtab\relax\else\global\tabprocessingfalse\fi
  \else
    \global\outputpretest={\outputtrue}%
  \fi
\fi
}
%----- hanging lord -----------------------------%
\def\dohang{%
   \dimen0=\fl@ht
   \advance\dimen0 by -\htdone
   \advance\dimen0 by 1.999\baselineskip	% (16/12/98) WAS 1.49 BUT
   \hangcount=\dimen0				% TEX ROUNDS ON STRICT INTEGERS
   \divide\hangcount by \baselineskip		% IN THIS DIVISION!
%	\typeout{HANGCOUNT: \the\hangcount.}
%   \ifnum\hangcount > 0	% IF ZERO ALSO INDENT MUST BE NULL. (7/6/97)
     \dimen0=\fl@wd
     \advance\dimen0 by \fl@gut
     \ifoddpages
       \global\hangindent=-\dimen0% placing right
     \else 
       \global\hangindent=\dimen0% placing left
     \fi
   \global\hangafter=-\hangcount
%   \fi
}
%----------------------- TWO NEWITEMS ---------------------%
\newcommand{\fltitem}[2][\z@]{\setlength{\fltitemwidth}{\linewidth}%
  \addtolength{\fltitemwidth}{-\floatfltwidth}%
  \addtolength{\fltitemwidth}{-0.5em}%
  \item \parbox[t]{\fltitemwidth}{#2}\\[#1]}
\newcommand{\fltditem}[3][\z@]{\setlength{\fltitemwidth}{\linewidth}%
  \addtolength{\fltitemwidth}{-\floatfltwidth}%
  \addtolength{\fltitemwidth}{-0.5em}%
  \item[#2] \parbox[t]{\fltitemwidth}{#3}\\[#1]}
%%%%%%\endinput
%% 
%% End of ex-file `floatflt.sty'.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CAPTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength\abovecaptionskip
\newlength\belowcaptionskip
\setlength\abovecaptionskip{8\p@}
\setlength\belowcaptionskip{0\p@}
\long\def\@makecaption#1#2{%
  \if@hyper{\edef\@pippo{the\@captype}
	    \name{\@captype\expandafter\csname\@pippo\endcsname}}\fi%
  \vskip\abovecaptionskip
 {\let\label\@gobble%				% FN 10.2.97 REMOVED LATEX BUG:
  \let\index\@gobble%				% LARGE CAPTIONS PROCESS LABEL
  \let\glossary\@gobble%			% TWO TIMES.
  \sbox\@tempboxa{\small {\bfseries #1:} #2}%	% 
  \global\dimen0\wd\@tempboxa}%			%
  \ifdim \dimen0 >\hsize
    \small {\bfseries #1:} #2\par
  \else
    \global\@minipagefalse \sbox\@tempboxa{\small {\bfseries #1:} #2}%
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FONTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}
\DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}
\DeclareRobustCommand*\mit{\@fontswitch\relax\mathnormal}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TOC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\tocsecs{}
\newcommand\@pnumwidth{1.55em}
\newcommand\@tocrmarg{2.55em}
\newcommand\@dotsep{4.5}
\setcounter{tocdepth}{3}
\newcommand\tableofcontents{%
    \section*{\contentsname\label{-TOC-}}
%        \@mkboth{%
%           \MakeUppercase\contentsname}{\MakeUppercase\contentsname}%
    \@starttoc{toc}%
    \gdef\tableofcontents{\JHEP@igno{\tableofcontents\space already done}}}
\newcommand*\l@part[2]{\def\hyp@typ{part}%	
  \ifnum \c@tocdepth >-2\relax
    \addpenalty\@secpenalty
    \addvspace{2.25em \@plus\p@}%
    \begingroup
      \setlength\@tempdima{3em}%
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      {\leavevmode
       \large \bfseries \tocsecs#1\hfil \hb@xt@\@pnumwidth{\hss
		\intJlink{\hash pag#2}{#2}}}\par
       \nobreak
       \if@compatibility
         \global\@nobreaktrue
         \everypar{\global\@nobreakfalse\everypar{}}%
      \fi
    \endgroup
  \fi}
\newcommand*\l@section[2]{\def\hyp@typ{sec}%
  \ifnum \c@tocdepth >\z@
    \addpenalty\@secpenalty
    \addvspace{1.0em \@plus\p@}%
    \setlength\@tempdima{1.8em}%	%WIDTH OF SECT. N.
    \begingroup
      \let\d@t.%
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      \leavevmode \bfseries
      \advance\leftskip\@tempdima
      \hskip -\leftskip
        \tocsecs#1\nobreak\hfil %HREF HERE WOULD GET ALSO THE TITLE(...)
        \nobreak\hb@xt@\@pnumwidth{\hss \intJlink{\hash pag#2}{#2}}\par
    \endgroup
  \fi}

\newcommand*\l@subsection{\def\hyp@typ{sec}\@tocline{2}{1.8em}{2.3em}}
\newcommand*\l@subsubsection{\def\hyp@typ{sec}\@tocline{3}{4.1em}{3.1em}}
\newcommand*\l@paragraph{\def\hyp@typ{sec}\@tocline{4}{7.2em}{4.3em}}
\newcommand*\l@subparagraph{\def\hyp@typ{sec}\@tocline{5}{10.5em}{5em}}

\if@hyper
  \let\old@dtl\@dottedtocline
  \def\@dottedtocline#1#2#3#4#5{\old@dtl{#1}{#2}{#3}{#4}{%
						\intJlink{\hash pag#5}{#5}}}
\fi

\def\@tocline#1#2#3#4#5{%
  \ifnum #1>\c@tocdepth \else
    \vskip \z@ \@plus.2\p@
    {\leftskip #2\relax \rightskip \@tocrmarg \parfillskip -\rightskip
     \parindent #2\relax\@afterindenttrue
     \interlinepenalty\@M
     \leavevmode
     \@tempdima #3\relax
     \advance\leftskip \@tempdima \null\nobreak\hskip -\leftskip
     {#4}\nobreak
     %\leaders\hbox{$\m@th
     %   \mkern \@dotsep mu\hbox{.}\mkern \@dotsep
     %	   mu$}
     \hfill
     \nobreak
     \hb@xt@\@pnumwidth{\hfil\normalfont \normalcolor \intJlink{\hash pag#5}{#5}}%
     \par}%
  \fi}


%%%%%%%%%%%%%%%%%%%%%% LIST OF FIGURES AND TABLES %%%%%%%%%%%%%%%%%%%%%
\if@draft			% ONLY IF DRAFT! ... 
 \newcommand\listoffigures{%
     \section*{\listfigurename
       \@mkboth{\MakeUppercase\listfigurename}%
               {\MakeUppercase\listfigurename}}%
     \@starttoc{lof}%
     }
 \newcommand*\l@figure{\def\hyp@typ{figure}\@dottedtocline{1}{1.5em}{2.3em}}
 \newcommand\listoftables{%
     \section*{\listtablename
       \@mkboth{%
           \MakeUppercase\listtablename}{\MakeUppercase\listtablename}}%
     \@starttoc{lot}%
     }
 \newcommand*\l@table{\def\hyp@typ{table}\@dottedtocline{1}{1.5em}{2.3em}}
\else
 \newcommand\listoffigures{\JHEP@ignol{List of figures (draft mode only)}}
 \newcommand\listoftables{\JHEP@ignol{List of tables (draft mode only)}}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BIBLIOGRAPHY %%%%%%%%%%%%%%%%%%%%%%%%%%%%***
\newdimen\bibindent
\setlength\bibindent{1.5em}
\newenvironment{thebibliography}[1]%	%UNFORTUNATELY MODIFIED..
     {\bgroup\raggedright\small\section*{\refname
        \@mkboth{\MakeUppercase\refname}{\MakeUppercase\refname}}%
      \list{\name{bib\@arabic\c@enumiv}% HOPE!
	    \@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy\clubpenalty4000\widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist\egroup}
\newcommand\newblock{\hskip .11em\@plus.33em\@minus.07em}
\if@draft
 \let\old@bbt\@bibitem\let\old@lbbt\@lbibitem% LOOK THE DISASTER HERE BELOW.
 \def\@lbibitem[#1]#2{\old@lbbt[#1]{#2}\reversemarginpar{\sf\bfseries\small#2}}
 \def\@bibitem#1{\old@bbt{#1}\reversemarginpar{\sf\bfseries\small#1}}
\fi
\let\@openbib@code\@empty
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% JOURNALS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@spires#1{\href{http://www-spires.slac.stanford.edu/spires/find/hep/www?j=#1}} 
%                               	%PITY THAT target IS NOT IMPLEMENTED.
\catcode`\%=12
\catcode`\|=14
\newcommand\apa[3]    {\@spires{APASA%2C#1%2C#3}
		{{\it Acta Phys.\ Austriaca }{\bf #1} (#2) #3}}
\newcommand\apas[3]    {\@spires{APAUA%2C#1%2C#3}
		{{\it Acta Phys.\ Austriaca, Suppl.\ }{\bf #1} (#2) #3}}
\newcommand\appol[3] {\@spires{APPOA%2C#1%2C#3}
		{{\it Acta Phys.\ Polon.\ }{\bf #1} (#2) #3}}
\newcommand\advm[3]  {\@spires{ADMTA%2C#1%2C#3}
		{{\it Adv.\ Math.\ }{\bf #1} (#2) #3}}
\newcommand\adnp[3]   {\@spires{ANUPB%2C#1%2C#3}
		{{\it Adv.\ Nucl.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\adp[3]   {\@spires{ADPHA%2C#1%2C#3}
		{{\it Adv.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\atmp[3] {\@spires{00203%2C#1%2C#3}
		{{\it Adv.\ Theor.\ Math.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\am[3]    {\@spires{ANMAA%2C#1%2C#3}
		{{\it Ann.\ Math.\ }{\bf #1} (#2) #3}}
\newcommand\ap[3]    {\@spires{APNYA%2C#1%2C#3}
		{{\it Ann.\ Phys.\ (NY) }{\bf #1} (#2) #3}}
\newcommand\araa[3] {\@spires{ARAAA%2C#1%2C#3}
		{{\it Ann.\ Rev.\ Astron.\ \& Astrophys.\ }{\bf #1} (#2) #3}}
\newcommand\arnps[3] {\@spires{ARNUA%2C#1%2C#3}
		{{\it Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ }{\bf #1} (#2) #3}}
\newcommand\asas[3]   {\@spires{AAEJA%2C#1%2C#3}
		{{\it Astron.\ Astrophys.\ }{\bf #1} (#2) #3}}
\newcommand\asj[3]   {\@spires{ANJOA%2C#1%2C#3}
		{{\it Astron.\ J.\ }{\bf #1} (#2) #3}}
\newcommand\app[3]   {\@spires{APHYE%2C#1%2C#3}
		{{\it Astropart.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\apj[3]    {\@spires{ASJOA%2C#1%2C#3}
		{{\it Astrophys.\ J. }{\bf #1} (#2) #3}}
\newcommand\baas[3]   {\@spires{AASBA%2C#1%2C#3}
		{{\it Bull.\ Am.\ Astron.\ Soc.\ }{\bf #1} (#2) #3}}
\newcommand\bams[3]   {\@spires{BAMOA%2C#1%2C#3}
		{{\it Bull.\ Am.\ Math.\ Soc.\ }{\bf #1} (#2) #3}}
\newcommand\blms[3]   {\@spires{LMSBB%2C#1%2C#3}
		{{\it Bull.\ London Math.\ Soc.\ }{\bf #1} (#2) #3}}
\newcommand\cjm[3]  {\@spires{CJMAA%2C#1%2C#3}
		{{\it Can.\ J.\ Math.\ }{\bf #1} (#2) #3}}
\newcommand\cqg[3]   {\@spires{CQGRD%2C#1%2C#3}
		{{\it Class.\ and Quant.\ Grav.\ }{\bf #1} (#2) #3}}
\newcommand\cmp[3]   {\@spires{CMPHA%2C#1%2C#3}
		{{\it Commun.\ Math.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\ctp[3]   {\@spires{CTPMD%2C#1%2C#3}
		{{\it Commun.\ Theor.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\cag[3]   {\@spires{00142%2C#1%2C#3}
		{{\it Commun.\ Anal.\ Geom.\ }{\bf #1} (#2) #3}}
\newcommand\cpam[3]   {\@spires{CPAMA%2C#1%2C#3}
		{{\it Commun.\ Pure Appl.\ Math.\ }{\bf #1} (#2) #3}}
\newcommand\cpc[3]   {\@spires{CPHCB%2C#1%2C#3}
		{{\it Comput.\ Phys.\ Commun.\ }{\bf #1} (#2) #3}}
\newcommand\dmj[3]   {\@spires{DUMJA%2C#1%2C#3}
		{{\it Duke Math.\ J. }{\bf #1} (#2) #3}}
\newcommand\epjc[3]  {\@spires{EPHJA%2CC#1%2C#3}
		{{\it Eur.\ Phys.\ J. }{\bf C #1} (#2) #3}}
\newcommand\epjd[3]  {\@spires{EPHJD%2CC#1%2C#3}
		{{\it Eur.\ Phys.\ J. Direct.\ }{\bf C #1} (#2) #3}}
\newcommand\epl[3]    {\@spires{EULEE%2C#1%2C#3}
		{{\it Europhys.\ Lett. }{\bf #1} (#2) #3}}
\newcommand\forp[3]    {\@spires{FPYKA%2C#1%2C#3}
		{{\it Fortschr.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\faa[3]    {\@spires{FAAPB%2C#1%2C#3}
		{{\it Funct.\ Anal.\ Appl.\ }{\bf #1} (#2) #3}}
\newcommand\grg[3]    {\@spires{GRGVA%2C#1%2C#3}
		{{\it Gen.\ Rel.\ Grav.\ }{\bf #1} (#2) #3}}
\newcommand\hpa[3]   {\@spires{HPACA%2C#1%2C#3}
		{{\it Helv.\ Phys.\ Acta }{\bf #1} (#2) #3}}
\newcommand\ijmpa[3] {\@spires{IMPAE%2CA#1%2C#3}
		{{\it Int.\ J.\ Mod.\ Phys.\ }{\bf A #1} (#2) #3}}
\newcommand\ijmpb[3] {\@spires{IMPAE%2CB#1%2C#3}
		{{\it Int.\ J.\ Mod.\ Phys.\ }{\bf B #1} (#2) #3}}
\newcommand\ijmpc[3] {\@spires{IMPAE%2CC#1%2C#3}
		{{\it Int.\ J.\ Mod.\ Phys.\ }{\bf C #1} (#2) #3}}
\newcommand\ijmpd[3] {\@spires{IMPAE%2CD#1%2C#3}
		{{\it Int.\ J.\ Mod.\ Phys.\ }{\bf D #1} (#2) #3}}
\newcommand\ijtp[3] {\@spires{IJTPB%2CB#1%2C#3}
		{{\it Int.\ J.\ Theor.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\invm[3]  {\@spires{INVMB%2C#1%2C#3}
		{{\it Invent.\ Math.\ }{\bf #1} (#2) #3}}
\newcommand\jag[3]   {\@spires{00124%2C#1%2C#3}
		{{\it J.\ Alg.\ Geom.\ }{\bf #1} (#2) #3}}
\newcommand\jams[3]   {\@spires{00052%2C#1%2C#3}
		{{\it J.\ Am.\ Math.\ Soc.\ }{\bf #1} (#2) #3}}
\newcommand\jap[3]   {\@spires{JAPIA%2C#1%2C#3}
		{{\it J.\ Appl.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\jdg[3]   {\@spires{JDGEA%2C#1%2C#3}
		{{\it J.\ Diff.\ Geom.\ }{\bf #1} (#2) #3}}
\newcommand\jgp[3]   {\@spires{JGPHE%2C#1%2C#3}
		{{\it J.\ Geom.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\jhep[3]  {\href{http://jhep.sissa.it/stdsearch?paper=#1%28#2%29#3}
		{{\it J. High Energy Phys.\ }{\bf #1} (#2) #3}}
\newcommand\jmp[3]   {\@spires{JMAPA%2C#1%2C#3}
		{{\it J.\ Math.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\joth[3]  {\@spires{JOTHE%2C#1%2C#3}
		{{\it J.\ Operator Theory }{\bf #1} (#2) #3}}
\newcommand\jpha[3]   {\@spires{JPAGB%2CA#1%2C#3}
		{{\it J. Phys.\ }{\bf A #1} (#2) #3}}
\newcommand\jphc[3]   {\@spires{JPAGB%2CC#1%2C#3}
		{{\it J. Phys.\ }{\bf C #1} (#2) #3}}
\newcommand\jphg[3]   {\@spires{JPAGB%2CG#1%2C#3}
		{{\it J. Phys.\ }{\bf G #1} (#2) #3}}
\newcommand\lmp[3]   {\@spires{LMPHD%2CA#1%2C#3}
		{{\it Lett.\ Math.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\ncl[3]    {\@spires{NCLTA%2C#1%2C#3}
		{{\it Lett.\ Nuovo Cim.\ }{\bf #1} (#2) #3}}
\newcommand\matan[3]  {\@spires{MAANA%2CA#1%2C#3}
		{{\it Math.\ Ann.\ }{\bf #1} (#2) #3}}
\newcommand\mussr[3]  {\@spires{MUSIA%2CA#1%2C#3}
		{{\it Math.\ USSR Izv.\ }{\bf #1} (#2) #3}}
\newcommand\mams[3]  {\@spires{MAMCA%2CA#1%2C#3}
		{{\it Mem.\ Am.\ Math.\ Soc.\ }{\bf #1} (#2) #3}}
\newcommand\mpla[3]  {\@spires{MPLAE%2CA#1%2C#3}
		{{\it Mod.\ Phys.\ Lett.\ }{\bf A #1} (#2) #3}}
\newcommand\mplb[3]  {\@spires{MPLAE%2CB#1%2C#3}
		{{\it Mod.\ Phys.\ Lett.\ }{\bf B #1} (#2) #3}}
\newcommand\nature[3]  {\@spires{NATUA%2C#1%2C#3}
		{{\it Nature }{\bf #1} (#2) #3}}
\newcommand\nim[3]   {\@spires{NUIMA%2C#1%2C#3}
		{{\it Nucl.\ Instrum.\ Meth.\ }{\bf #1} (#2) #3}}
\newcommand\npa[3]   {\@spires{NUPHA%2CA#1%2C#3}
		{{\it Nucl.\ Phys.\ }{\bf A #1} (#2) #3}}
\newcommand\npb[3]    {\@spires{NUPHA%2CB#1%2C#3}
		{{\it Nucl.\ Phys.\ }{\bf B #1} (#2) #3}}
\newcommand\npps[3]  {\@spires{NUPHZ%2C#1%2C#3}
		{{\it Nucl.\ Phys.\ }{\bf #1} {\it(Proc.\ Suppl.)} (#2) #3}}
\newcommand\nc[3]    {\@spires{NUCIA%2C#1%2C#3}
		{{\it Nuovo Cim.\ }{\bf #1} (#2) #3}}
\newcommand\ncs[3]  {\@spires{NUCUA%2C#1%2C#3}
		{{\it Nuovo Cim.\ Suppl.\ }{\bf #1} (#2) #3}}
\newcommand\pan[3]  {\@spires{PANUE%2C#1%2C#3}
		{{\it Phys.\ Atom.\ Nucl.\ }{\bf #1} (#2) #3}}
\newcommand\pla[3]   {\@spires{PHLTA%2CA#1%2C#3}
		{{\it Phys.\ Lett.\ }{\bf A #1} (#2) #3}}
\newcommand\plb[3]   {\@spires{PHLTA%2CB#1%2C#3}
		{{\it Phys.\ Lett.\ }{\bf B #1} (#2) #3}}
\newcommand\pr[3]    {\@spires{PHRVA%2C#1%2C#3}
		{{\it Phys.\ Rev.\ }{\bf #1} (#2) #3}}
\newcommand\pra[3]   {\@spires{PHRVA%2CA#1%2C#3}
		{{\it Phys.\ Rev.\ }{\bf A #1} (#2) #3}}
\newcommand\prb[3]   {\@spires{PHRVA%2CB#1%2C#3}
		{{\it Phys.\ Rev.\ }{\bf B #1} (#2) #3}}
\newcommand\prc[3]   {\@spires{PHRVA%2CC#1%2C#3}
		{{\it Phys.\ Rev.\ }{\bf C #1} (#2) #3}}
\newcommand\prd[3]   {\@spires{PHRVA%2CD#1%2C#3}
		{{\it Phys.\ Rev.\ }{\bf D #1} (#2) #3}}
\newcommand\pre[3]   {\@spires{PHRVA%2CE#1%2C#3}
		{{\it Phys.\ Rev.\ }{\bf E #1} (#2) #3}}
\newcommand\prep[3]  {\@spires{PRPLC%2C#1%2C#3}
		{{\it Phys.\ Rept.\ }{\bf #1} (#2) #3}}
\newcommand\prl[3]   {\@spires{PRLTA%2C#1%2C#3}
		{{\it Phys.\ Rev.\ Lett.\ }{\bf #1} (#2) #3}}
\newcommand\phys[3]   {\@spires{PHYSA%2CA#1%2C#3}
		{{\it Physica }{\bf #1} (#2) #3}}
\newcommand\plms[3]   {\@spires{PHLTA%2CB#1%2C#3}
		{{\it Proc.\ London Math.\ Soc.\ }{\bf B #1} (#2) #3}}
\newcommand\pnas[3]  {\@spires{PNASA%2C#1%2C#3}
		{{\it Proc.\ Nat.\ Acad.\ Sci.\ }{\bf #1} (#2) #3}}
\newcommand\ppnp[3]  {\@spires{PPNPD%2C#1%2C#3}
		{{\it Prog.\ Part.\ Nucl.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\ptp[3]   {\@spires{PTPKA%2C#1%2C#3}
		{{\it Prog.\ Theor.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\ptps[3]   {\@spires{PTPSA%2C#1%2C#3}
		{{\it Prog.\ Theor.\ Phys.\ Suppl.\ }{\bf #1} (#2) #3}}
\newcommand\rmp[3]   {\@spires{RMPHA%2C#1%2C#3}
		{{\it Rev.\ Mod.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\sjnp[3]  {\@spires{SJNCA%2C#1%2C#3}
		{{\it Sov.\ J.\ Nucl.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\sjpn[3]  {\@spires{SJPNA%2C#1%2C#3}
		{{\it Sov.\ J.\ Part.\ Nucl.\ }{\bf #1} (#2) #3}}
\newcommand\jetp[3]  {\@spires{SPHJA%2C#1%2C#3}
		{{\it Sov.\ Phys.\ JETP\/ }{\bf #1} (#2) #3}}
\newcommand\jetpl[3]  {\@spires{JTPLA%2C#1%2C#3}
		{{\it Sov.\ Phys.\ JETP Lett.\ }{\bf #1} (#2) #3}}
\newcommand\spu[3]  {\@spires{SOPUA%2C#1%2C#3}
		{{\it Sov.\ Phys.\ Usp.\ }{\bf #1} (#2) #3}}
\newcommand\tmf[3]   {\@spires{TMFZA%2C#1%2C#3}
		{{\it Teor.\ Mat.\ Fiz.\ }{\bf #1} (#2) #3}}
\newcommand\tmp[3]   {\@spires{TMPHA%2C#1%2C#3}
		{{\it Theor.\ Math.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\ufn[3]   {\@spires{UFNAA%2C#1%2C#3}
		{{\it Usp.\ Fiz.\ Nauk.\ }{\bf #1} (#2) #3}}
| }}}}}}}}}}}}}}}}}}}}}} "|" is here a comment (catcode defined above) to
| }}}}}}}}}}}}}}}}}}}}}} include parenthesis for emacs to parse properly. 
\newcommand\ujp[3]   {\@spires{00267%2C#1%2C#3}
		{{\it Ukr.\ J.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\yf[3]    {\@spires{YAFIA%2C#1%2C#3}
		{{\it Yad.\ Fiz.\ }{\bf #1} (#2) #3}}
\newcommand\zpc[3]   {\@spires{ZEPYA%2CC#1%2C#3}
		{{\it Z.\ Physik }{\bf C #1} (#2) #3}}
\newcommand\zetf[3]  {\@spires{ZETFA%2C#1%2C#3}
		{{\it Zh.\ Eksp.\ Teor.\ Fiz.\ }{\bf #1} (#2) #3}}

\newcommand{\newjournal}[5]{\@spires{#2%2C#3%2C#5}
		{{\it #1 }{\bf #3} (#4) #5}}

\newcommand\ibid[3]{{\it ibid.\ }{\bf #1} (#2) #3}
\catcode`\%=14
\catcode`\|=12
% HEPTH's: \hepth{9912999} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hepth}[1]{\href{http://xxx.lanl.gov/abs/hep-th/#1}{\tt hep-th/#1}}
\newcommand{\hepph}[1]{\href{http://xxx.lanl.gov/abs/hep-ph/#1}{\tt hep-ph/#1}}
\newcommand{\heplat}[1]{\href{http://xxx.lanl.gov/abs/hep-lat/#1}{\tt hep-lat/#1}}
\newcommand{\hepex}[1]{\href{http://xxx.lanl.gov/abs/hep-ex/#1}{\tt hep-ex/#1}}
\newcommand{\nuclth}[1]{\href{http://xxx.lanl.gov/abs/nucl-th/#1}{\tt nucl-th/#1}}
\newcommand{\nuclex}[1]{\href{http://xxx.lanl.gov/abs/nucl-ex/#1}{\tt nucl-ex/#1}}
\newcommand{\grqc}[1]{\href{http://xxx.lanl.gov/abs/gr-qc/#1}{\tt gr-qc/#1}}
\newcommand{\qalg}[1]{\href{http://xxx.lanl.gov/abs/q-alg/#1}{\tt q-alg/#1}}
\newcommand{\accphys}[1]{\href{http://xxx.lanl.gov/abs/accphys/#1}{\tt accphys/#1}}
\newcommand{\alggeom}[1]{\href{http://xxx.lanl.gov/abs/alg-geom/#1}{\tt alg-geom/#1}}
\newcommand{\astroph}[1]{\href{http://xxx.lanl.gov/abs/astro-ph/#1}{\tt astro-ph/#1}}
\newcommand{\chaodyn}[1]{\href{http://xxx.lanl.gov/abs/chao-dyn/#1}{\tt chao-dyn/#1}}
\newcommand{\condmat}[1]{\href{http://xxx.lanl.gov/abs/cond-mat/#1}{\tt cond-mat/#1}}
\newcommand{\nlinsys}[1]{\href{http://xxx.lanl.gov/abs/nlin-sys/#1}{\tt nlin-sys/#1}}
\newcommand{\quantph}[1]{\href{http://xxx.lanl.gov/abs/quant-ph/#1}{\tt quant-ph/#1}}
\newcommand{\solvint}[1]{\href{http://xxx.lanl.gov/abs/solv-int/#1}{\tt solv-int/#1}}
\newcommand{\suprcon}[1]{\href{http://xxx.lanl.gov/abs/supr-con/#1}{\tt supr-con/#1}}
%\newcommand{\mathph}[1]{\href{http://xxx.lanl.gov/abs/math-ph/#1}{\tt math-ph/#1}}
%\newcommand{\physics}[1]{\href{http://xxx.lanl.gov/abs/physics/#1}{\tt physics/#1}}
\newcommand{\Math}[2]{\href{http://xxx.lanl.gov/abs/math.#1/#2}{\tt math.#1/#2}}
\newcommand{\arXivid}[1]{\href{http://arxiv.org/abs/#1}{\tt arXiv:#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BopHook %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\if@preprint\else
\if@proc
\newcommand\PrHEP[1]{\@JHEPtrue\special{!userdict begin
/iseven {dup dup 2 idiv 2 mul eq} bind def
/BHend {
  translate rotate 
/Courier findfont 30 scalefont setfont 
0 0  moveto 0.80 setgray (#1) show grestore}
 bind def
statusdict /duplexmode known 
  {statusdict begin duplexmode end}
  {false}
ifelse
  {/bop-hook {gsave iseven {-90 550 570} {+90 50 300} ifelse BHend} def}
  {/bop-hook {gsave         -90 550 570                      BHend} def}
ifelse 
end
}\let\PrHEP\gobble}\else
\newcommand\JHEP[1]{\Jsplit@ident#1.\@JHEPtrue\special{!userdict begin
/iseven {dup dup 2 idiv 2 mul eq} bind def
/BHend {
  translate rotate 
/Courier findfont 30 scalefont setfont 
0 0  moveto 0.80 setgray (JHEP#1) show grestore}
 bind def
statusdict /duplexmode known 
  {statusdict begin duplexmode end}
  {false}
ifelse
  {/bop-hook {gsave iseven {-90 550 570} {+90 50 300} ifelse BHend} def}
  {/bop-hook {gsave         -90 550 570                      BHend} def}
ifelse 
end
}\let\JHEP\gobble}\fi
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% INDEX %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%..?
%                          	% REMOVED
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FOOTNOTES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\skip\footins = 1\bigskipamount plus 2pt minus 8pt

\addtolength{\footnotesep}{1pt}
\renewcommand\footnoterule{%	% NO HYPER...
  \kern-3\p@
  \hrule\@width.4\columnwidth
  \kern2.6\p@}
\newcommand\@makefntext[1]{%
    \parindent 1em%
    \noindent
    \hb@xt@1.8em{\hss\@makefnmark}#1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NAMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\contentsname{Contents}
\if@draft\newcommand\listfigurename{List of figures}
	 \newcommand\listtablename{List of tables}\fi
\newcommand\refname{References}
\newcommand\indexname{Index}
\newcommand\figurename{Figure}
\newcommand\tablename{Table}
\newcommand\partname{Part}
\newcommand\appendixname{Appendix}
\newcommand\abstractname{Abstract:}
\newcommand\keywordsname{Keywords:}
\newcommand\receivedname{Received:}
\newcommand\revisedname{Revised:}
\newcommand\acceptedname{Accepted:}
\newcommand\acknowlname{Acknowledgments}

\newcommand\today{}
\edef\today{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\day, \number\year}

\setlength\columnsep{20\p@}
\setlength\columnseprule{0\p@}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DEFAULTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\pagestyle{plain}
\pagestyle{JHEP}
\pagenumbering{arabic}
\@addtoreset{equation}{section}
\if@preprint\else\if@proc\else
		\let\pagestyle\@gobble
		\let\thispagestyle\@gobble
		\let\pagenumbering\@gobble\fi\fi
%\if@twoside\else\raggedbottom\fi
  \onecolumn
						
% FOR REQUESTED FRONTMATTER ...
\AtBeginDocument{\bgroup%		SOME NICE (LOCAL) MESSAGES... 
	\def\@APPwarn#1{\JHEP@warnl{\protect#1 should appear 
					before \protect\begin{document}}}%
	\def\@APPerr#1{\ClassError{JHEP}{\protect#1 should appear 
					before \protect\begin{document}}}%
%	\if@title\else\@APPerr{Some \protect\title{...}}\fi%
	\if@author\else\@APPerr{Some \protect\author{...}}\fi
	\if@abstract\else\@APPerr{\abstract{...}}\fi
%	\if@email\else\@APPwarn{\email}\fi%
	\if@proc\else\if@keywords\else\@APPwarn{\keywords{...}}\fi\fi
	\if@preprint
		\ifx\@preprint\relax\@APPwarn{\preprint{...}}\fi
	\else
		\if@proc\if@conf\else\@APPwarn{\conference{...}}\fi
		\else	\if@rece\else\@APPerr{\received{...}}\fi
			\if@acce\else\@APPerr{\accepted{...}}\fi
			\if@JHEP\else\@APPerr{\JHEP{mm(yyyy)nnn}}\fi
		\fi
	\fi
	\egroup
	\auto@maketitle
	\if@proc\if@speaker\else\JHEP@warnl{One \protect\speaker{...}
			must be specified among authors}\fi
			\if@dblspeak\JHEP@warnl{A single \protect\speaker{...}
			should appear in proceedings}\fi\fi
			}% IN THE BEGINNING THERE WAS THE TITLE, TYPESET IN TeX 
\endinput
%% 
%% End of file `JHEP3.cls'.

